Energy-adaptive Buffering for Efficient, Responsive, and Persistent Batteryless Systems

Batteryless energy harvesting systems enable a wide array of new sensing, computation, and communication platforms untethered by power delivery or battery maintenance demands. Energy harvesters charge a buffer capacitor from an unreliable environmental source until enough energy is stored to guarantee a burst of operation despite changes in power input. Current platforms use a fixed-size buffer chosen at design time to meet constraints on charge time or application longevity, but static energy buffers are a poor fit for the highly volatile power sources found in real-world deployments: fixed buffers waste energy both as heat when they reach capacity during a power surplus and as leakage when they fail to charge the system during a power deficit. To maximize batteryless system performance in the face of highly dynamic input power, we propose REACT: a responsive buffering circuit which varies total capacitance according to net input power. REACT uses a variable capacitor bank to expand capacitance to capture incoming energy during a power surplus and reconfigures internal capacitors to reclaim additional energy from each capacitor as power input falls. Compared to fixed-capacity systems, REACT captures more energy, maximizes usable energy, and efficiently decouples system voltage from stored charge -- enabling low-power and high-performance designs previously limited by ambient power. Our evaluation on real-world platforms shows that REACT eliminates the tradeoff between responsiveness, efficiency, and longevity, increasing the energy available for useful work by an average 25.6% over static buffers optimized for reactivity and capacity, improving event responsiveness by an average 7.7x without sacrificing capacity, and enabling programmer directed longevity guarantees.

==> Figures/background_comparison.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{3.65pt}
\centering
\footnotesize{}
\begin{tabular}{c|cccc}
                  & \textbf{\begin{tabular}[c]{@{}c@{}}Quick\\ Charge\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Dynamic\\ Prioritization\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Energy\\ Fungibility\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Efficient\\ Reconfig.\end{tabular}} \\ \hline
\textbf{UFoP~\cite{federation}}     & \checkmark                                                       & X                                                                         & X                                                                     & X                                                                     \\
\textbf{Flicker~\cite{flicker}}  & \checkmark                                                       & \checkmark                                                                 & X                                                                     & X                                                                     \\
\textbf{Dewdrop~\cite{dewdrop}}  & X                                                               & \checkmark                                                                 & \checkmark                                                             & \checkmark                                                                     \\
\textbf{Capybara~\cite{capybara}} & \checkmark                                                       & X                                                                         & X                                                                     & X                                                                     \\
\textbf{Morphy~\cite{morphy}}   & \checkmark                                                       & \checkmark                                                                 & \checkmark                                                             & X                                                                     \\ \hline
\textbf{\sys{}}    & \checkmark                                                       & \checkmark                                                                 & \checkmark                                                             & \checkmark                                                            
\end{tabular}
\caption{Comparison of \sys{} with related work exploring buffer behavior for batteryless systems.}
\label{table:background-comparison}
% \vspace{-2pt}
\hrulefill
\end{table}

==> Figures/basic_operation.tex <==
\begin{figure}[t]
 \centering
  \includegraphics[width=0.9\columnwidth]{Figures/basic_operation.pdf}
  \caption{Example of \sys{} expanding and contracting buffer capacitance during the RF Cart power trace.}
  \label{fig:basic-operation}
  \hrulefill
\end{figure}

==> Figures/benchmark_table.tex <==
\begin{table}[]
\setlength{\tabcolsep}{4.5pt}
\centering
\footnotesize{}
\begin{tabular}{c|cccc}
\textbf{Benchmark}       & \textbf{DE}  & \textbf{SC}   & \textbf{RT} & \textbf{PF}                 \\ \hline
\textbf{Avg. Power (mW)} & 0.748        & 0.138         & 17.5        & 1.24                        \\
\textbf{Peak Power (mW)} & 0.748        & 1.2           & 17.5        & 17.5                        \\
\textbf{Reactivity}      & Low          & High          & Low         & High                        \\
\textbf{Persistence}     & Low          & Low           & High        & High                        \\
\textbf{Figure of Merit} & Encryptions  & Samples       & Tx          & Rx, Tx
\end{tabular}
\caption{Evaluation benchmarks and performance metrics. Power measurements are taken on continuous power.}
\label{table:benchmarks}
\hrulefill
\end{table}

==> Figures/cost_table.tex <==
\begin{table}[]
\setlength{\tabcolsep}{3.75pt}
\renewcommand{\arraystretch}{0.95} % Default value: 1
\centering
\footnotesize{}
% \begin{tabular}{c|ccccc}
% \multirow{2}{*}{\textbf{Device}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}1000x\\ Unit Cost\end{tabular}}}} & \multicolumn{2}{c|}{\textbf{Morphy}} & \multicolumn{2}{c}{\textbf{REACT}} \\
%                                  & \multicolumn{1}{c|}{}                                                                                    & Count & \multicolumn{1}{c|}{Cost}    & Count      & Cost                  \\ \hline
% Supercap.~\cite{mySupercap}                        & \multicolumn{1}{c|}{\$1.54}                                                                              & 17    & \multicolumn{1}{c|}{\$26.19} & 16         & \$24.65               \\
% Switch IC~\cite{adg824}                        & \multicolumn{1}{c|}{\$1.53}                                                                              & 17    & \multicolumn{1}{c|}{\$26.01} & 12         & \$18.36               \\
% Ceramic Cap.~\cite{myCeramics}                     & \multicolumn{1}{c|}{\$0.45}                                                                              & 0     & \multicolumn{1}{c|}{\$0}     & 4          & \$1.82                \\
% Ideal Diode~\cite{lm66100}                      & \multicolumn{1}{c|}{\$0.27}                                                                              & 0     & \multicolumn{1}{c|}{\$0}     & 16         & \$4.32                \\
% Comparator IC~\cite{tlv7044}                    & \multicolumn{1}{c|}{\$0.77}                                                                              & 0     & \multicolumn{1}{c|}{\$0}     & 1          & \$0.77                \\
% Detector IC~\cite{bu49xx}                 & \multicolumn{1}{c|}{\$0.26}                                                                              & 0     & \multicolumn{1}{c|}{\$0}     & 2            & \$0.52              \\
% Control MCU~\cite{pic18lf65k40}                      & \multicolumn{1}{c|}{\$2.37}                                                                              & 1     & \multicolumn{1}{c|}{\$2.37}  & 0          & \$0                   \\
% RTC~\cite{ab0805}                              & \multicolumn{1}{c|}{\$1.08}                                                                              & 1     & \multicolumn{1}{c|}{\$1.08}  & 0          & \$0                   \\ \hline
% \textbf{Platform cost}           &                                                                                                          &       & \textbf{\$55.65}             &            & \textbf{\$50.44}     
% \end{tabular}
\begin{tabular}{c|ccccc}
\multirow{2}{*}{\textbf{Device}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}1000x\\ Unit Cost\end{tabular}}}} & \multicolumn{2}{c|}{\textbf{Morphy}} & \multicolumn{2}{c}{\textbf{REACT}} \\
                                 & \multicolumn{1}{c|}{}                                                                                    & Count & \multicolumn{1}{c|}{Cost}    & Count        & Cost                \\ \hline
Supercap.~\cite{mySupercap}      & \multicolumn{1}{c|}{\$1.54}                                                                              & 9     & \multicolumn{1}{c|}{\$13.87} & 8            & \$12.33             \\
Switch IC~\cite{adg824}          & \multicolumn{1}{c|}{\$1.53}                                                                              & 12    & \multicolumn{1}{c|}{\$18.36} & 6            & \$9.18              \\
Ideal Diode~\cite{lm66100}       & \multicolumn{1}{c|}{\$0.27}                                                                              & 1     & \multicolumn{1}{c|}{\$0.27}  & 8            & \$2.16              \\
Ceramic Cap.~\cite{myCeramics}   & \multicolumn{1}{c|}{\$0.45}                                                                              & 0     & \multicolumn{1}{c|}{\$0}     & 4            & \$1.82              \\
Comparator IC~\cite{tlv7044}     & \multicolumn{1}{c|}{\$0.77}                                                                              & 0     & \multicolumn{1}{c|}{\$0}     & 1            & \$0.77              \\
Detector IC~\cite{bu49xx}        & \multicolumn{1}{c|}{\$0.26}                                                                              & 0     & \multicolumn{1}{c|}{\$0}     & 2            & \$0.52              \\
Control MCU~\cite{pic18lf65k40}  & \multicolumn{1}{c|}{\$2.37}                                                                              & 1     & \multicolumn{1}{c|}{\$2.37}  & 0            & \$0                 \\
RTC~\cite{ab0805}                & \multicolumn{1}{c|}{\$1.08}                                                                              & 1     & \multicolumn{1}{c|}{\$1.08}  & 0            & \$0                 \\ \hline
\textbf{Platform Cost}           &                                                                                                          &       & \textbf{\$35.94}             & \textbf{}    & \textbf{\$26.77}   
\end{tabular}
\caption{Cost comparison between \sys{} and Morphy implementations targeting the same capacitance range.}
\label{table:cost-table}
\hrulefill
\end{table}

==> Figures/efficiency_curves.tex <==
\begin{figure}[t]
  \includegraphics[width=\columnwidth]{Figures/efficiency_curves.pdf}
  \caption{\footnotesize \hrw{Efficiency curves without a boost converter or current limiting.} \hrw{After thinking, probably remove. Dissipation is a giant mess. Maybe just keep voltage part and include $N=4$ for fun.} \hrw{Consider adding TPS63901 buck-boost line at 5.5V}}
  \label{fig:efficiency_curves}
  \hrulefill
\end{figure}

==> Figures/morphy_configs.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{Figures/morphy-configs-side.pdf}
  \caption{Morphy configurations we implement and evaluate. Not shown are four additional configurations where unused capacitors are increasingly connected in series.}
  \label{fig:morphy-configs}
  \hrulefill
\end{figure}

==> Figures/power_histogram.tex <==
\begin{figure}[t]
  \includegraphics[width=\columnwidth]{Figures/power_histogram.pdf}
  \caption{\footnotesize Histogram of harvested solar power compared to platform power levels. \hrw{Fix this to reflect changes in simulated solar harvester, see simulation.cpp} \hrw{Actually more likely just remove. Can describe what's going on in this picture in like 2 sentences}}
  \label{fig:power_histogram}
  \hrulefill
\end{figure}
% Source: portionFromTrace.py run on solar/mobile_trace.txt

==> Figures/system_photo.tex <==
\begin{figure}[t]
\centering
  \includegraphics[width=0.8\columnwidth]{Figures/system-photo.jpg}
  \caption{Breadboard implementations of \sys{}, the baseline Morphy system, and the power trace replay board.}
  \label{fig:system-photo}
  \hrulefill
\end{figure}

==> discussion.tex <==
\section{Discussion}

Energy harvesting applications that require extending programs across power failures longer than the SRAM remanence time pose a challenge to \sys{} because execution restarts from the beginning when SRAM data is lost.
However, these use cases are atypical and we expect \sys{} to be applicable in the majority of intermittent computation systems.
We discuss, but do not implement, methods for adapting \sys{} to systems that must continue computation across long power cycles.

\paragraph{Periodic NVM Checkpoints:}
One option to ensure a long-running computation survives arbitrary-length power cycles is to periodically write checkpoints to NVM.
Lightweight \sys{} checkpoints provide resilience to power cycles shorter than the SRAM remanence time, while slower NVM checkpoints ensure that some program progress is retained across longer power cycles.
The designer can balance execution overhead with guaranteed state retention by varying the frequency of NVM checkpoints.
For example, a Flash system that replaces 1 in 10 SRAM-based checkpoints with Mementos-style NVM checkpoints ensures the program makes some progress across power cycles of any length with approximately 10\% of the execution time overhead of a purely NVM-based checkpointing scheme.

\paragraph{Forward Progress Counters:}
Designers can also take a counter-based approach that records a non-volatile checkpoint when \sys{} checkpoints continuously fail to recover.
We envision such a system to operate in the following manner:
\begin{enumerate}
    \item Each time the recovery routine detects a corrupted SRAM file, increment a persistent counter.
    \item If the recovery routine successfully restores a checkpoint from the SRAM, reset the counter.
    \item Once the counter reaches a threshold value, indicating a certain number of failed SRAM checkpoints in a row, replace the next SRAM in-place checkpoint with an NVM-based checkpoint.
\end{enumerate}
This allows systems to adapt to changing power environments by depending primarily on low-overhead SRAM-based checkpoints when off times are short and falling back to NVM-based checkpoints when off times are too long to reliably retain data in SRAM.


==> main-old-jpaper.tex <==
% \documentclass[pageno]{jpaper}
% % \documentclass[sigconf,screen]{acmart}

% \usepackage{cite}
% \usepackage{amsmath,amssymb,amsfonts}
% \usepackage{algorithmic}
% \usepackage{graphicx}
% \usepackage{textcomp}
% \usepackage{xcolor}
% \usepackage{url}

% \newcommand{\ignore}[1]{}
% \newcommand{\ifspace}[1]{\ignore{}}

% \newcommand{\sys}{\textit{REACT}}
% \newcommand{\mytilde}{\raise.17ex\hbox{$\scriptstyle\mathtt{\sim}$}}
% \newcommand{\ie}{i.e.,}
% \newcommand{\eg}{e.g.,}

% \usepackage[normalem]{ulem}
% \usepackage{pifont}

% \usepackage{algorithm}
% \usepackage{tabularx}
% \usepackage{mathtools}
% \usepackage{subfig}
% \usepackage{colortbl}
% \usepackage{multirow}
% \usepackage[normalem]{ulem}

% \newcommand{\hrw}[1]{\textbf{\color{blue}[HRW: #1]}}
% % \newcommand{\mdh}[1]{\textbf{\color{purple}[MDH: #1]}}
% % \newcommand{\needref}{\textbf{[?]}}

% %replace XXX with the submission number you are given from the ASPLOS submission site.
% \newcommand{\asplossubmissionnumber}{916}

% \usepackage[normalem]{ulem}

% \begin{document}

% %%%% Keywords for system name
% % Flexible
% % Variable
% % Fluid
% % Dynamic
% % Adjustable
% % Fungible
% % Goldilocks
% % Fluid energy buffer
% % FittedCap
% % Elasticap
% % Elastcap
% % Dynamicap
% % Goldicaps
% % Graduated cap
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % Concept to remember wrt cold-start energy if a reviewer says "cold-start energy is a transient one-time cost you pay then it doesn't mean anything, leakage isn't that bad.
% % Your performance improvements are an artifact of fixed-length traces rather than the system actually running better"

% % Cite \ref{batteryless-ingestible}! Energy harvester that can harvest a fixed amount of energy (but power input still fits EH behavior: unpredictable, scarce, etc.
% % The anode dissolves in the electrolyte (stomach acid) to produce a current so you will never get it back.

% \title{
% Energy-Adaptive Buffering for Efficient, Responsive, and Persistent Batteryless Systems}

% \date{}
% \maketitle

% \thispagestyle{empty}

% \input{abstract.tex}

% % \thispagestyle{empty}

% \input{introduction.tex}

% \input{background.tex}

% %\input{problem.tex}

% % \input{motivation.tex}

% \input{design.tex}

% \input{implementation.tex}

% \input{evaluation.tex}

% \ifspace{
% \input{discussion.tex}
% }

% % \input{related.tex}

% \input{conclusion.tex}

% \bibliographystyle{plain}
% \bibliography{refs}

% \input{appendix.tex}

% \end{document}


==> motivation.tex <==
\section{Motivation}
Motivation

==> problem.tex <==
\section{Problem}

To enable reliable intermittent computing, 
prior works propose checkpointing program state to NVM prior to power failure and restoring the checkpointed program state from NVM after powering on \cite{}.  Checkpointing to Flash is costly because  checkpointing is write-intensive and writes are costly under Flash (see Section \ref{sec:NVM_tradeoff}). Our real-system evaluation (see Section \ref{sec:methodology} for detailed methodology) using an MSP430 operating at ??MHz shows that writing a 2KB (i.e., MSP430's SRAM size \cite{}) checkpoint to Flash requires a total of ??ms. Figure \ref{fig:} sweeps the runtime overhead of checkpointing 2KB to Flash for different durations of microcontroller on time. Assuming an on time of ??ms used in prior work \cite{}, checkpointing 2KB of program memory from SRAM to Flash before every power failure translates to ??\% of runtime overhead. Assuming a shorter on time of ??ms used in  \cite{}, checkpointing 2KB of data to Flash is impossible because checkpointing to Flash takes longer than on time! While allocating the memory heap and stack entirely in NVM, instead of SRAM, can eliminate the need to checkpoint 2KB of SRAM content to Flash at the end of each power cycle, writing continuously to Flash can severely reduce Flash lifetime; assuming a Flash erase/write cycle of ?? \cite{}, a Flash capacity of ??KB (i.e.,  MSP430's Flash size \cite{}), and an conservative average write rate of ??times/second to Flash-allocated memory stack and heap,  a section of Flash memory will become unusable within two days. Mementos~\cite{mementos}, a state-of-art prior work that checkpoints to Flash when power failure is imminent, also reports 65\% to 360\% execution time overhead and does not address the endurance problem.

To address the high checkpointing overheads to Flash, prior works  have explored microcontrollers with FRAM~\cite{quickrecall, ratchet, hibernus}. For example, Hibernus~\cite{hibernus}, a state-of-the-art FRAM checkpointing system, applies Mementos's approach to systems with FRAM NVM and achieves 20\% time and energy overhead in similar test conditions. However, microcontrollers with FRAM suffer from many factors of density loss and monetary cost compared to microcontrollers with Flash (see Section \ref{sec:tradeoff}). While prior works have also proposed using alternative NVM technologies, such as MRAMs \cite{nvp_mram}, these memories are still in the experimental/prototyping stage. Even if emerging NVM technologies do achieve mass production, incorporating them into existing microcontrollers still requires non-trivial hardware integration and verification. Ideally, we want to enable efficient checkpointing for \emph{existing COTS} microcontrollers with Flash to avoid the low-density and cost problems of FRAM and the uncertainty of and long wait for incorporating emerging NVMs; this is the goal of this paper.  


==> related.tex <==
\section{Related Work}
Related work
